FewNLU: Benchmarking State-of-the-Art Methods for Few-Shot Natural Language Understanding

The few-shot natural language understanding (NLU) task has attracted much recent attention. However, prior methods have been evaluated under a disparate set of protocols, which hinders fair comparison and measuring progress of the field. To address this issue, we introduce an evaluation framework that improves previous evaluation procedures in three key aspects, i.e., test performance, dev-test correlation, and stability. Under this new evaluation framework, we re-evaluate several state-of-the-art few-shot methods for NLU tasks. Our framework reveals new insights: (1) both the absolute performance and relative gap of the methods were not accurately estimated in prior literature; (2) no single method dominates most tasks with consistent performance; (3) improvements of some methods diminish with a larger pretrained model; and (4) gains from different methods are often complementary and the best combined model performs close to a strong fully-supervised baseline. We open-source our toolkit, FewNLU, that implements our evaluation framework along with a number of state-of-the-art methods.

==> 3_3_which_hyperparameters.tex <==
\subsection{Which Hyper-Parameters are Crucial}\label{sec:howtosearchparam}


\subsubsection{Should We Search Random Seeds?}\label{sec:keyfactor}

In this work, we focus on two types of factors that affect few-shot evaluation, hyper-parameters and randomness.
Randomness could cause different weight initialization, data splits, and data order during training.
Empirically, how randomness is dealt with differs depending on the use case. In order to obtain the best possible performance, one could search over sensitive random factors such as random seeds.
However, as we are focused on benchmarking few-shot NLU methods, we report mean results (along with the standard deviation) in our experiments in order to rule out the effects of randomness and reflect the average performance of a method for fair comparison and measurement.


\subsubsection{Experiments}\label{sec:crucialhyperparam}

\paragraph{Experimental Setup}

To examine how a certain factor affects few-shot performance,
we assign multiple different values to a target factor while fixing other hyper-parameters. 
% we conduct experiments by assigning different values to a target factor and fixing all other hyper-parameters. 
We report the standard deviation over the multiple results.
Larger values indicate that a perturbation of the target factor would largely influence the few-shot performance and the factor thus is crucial for searching.
We experiment on BoolQ, RTE, CB, and COPA tasks.
Considered factors include: sample order during training, prompt pattern, training batch size, learning rate, evaluation frequency, and maximum train steps.
% ~\footnote{Note that we only want to explore the stability under a small disturbance, so we don't consider extreme values, which certainly will make the model fail and thus does not make much sense practically.}
More experimental details are in Appendix~\ref{apdx:part2_details}.
\input{latex/tables/setting_crucial_hparams}

\paragraph{Results and Analysis}
Results are in Table~\ref{tab:factors}. We mark values larger than a threshold of $2.0$ in bold.
We can see that the prompt pattern is the most influential factor among all, indicating the design or selection of prompt patterns is crucial.
Training example order also significantly affects the performance.
The evaluation frequency affects the score on the small development but not on the test set. 
We speculate that a lower frequency selects a model with better performance on the small development set, but the gains do not transfer to the test set because of partial overfitting. To conclude:
\begin{theorem}\label{thm:crucialfactor}
We recommend to at least search over prompt patterns during hyper-parameter tuning, and it is also beneficial to search others.
All comparison methods should be searched and compared under the same set of hyper-parameters.
% The same set of hyper-parameters should be searched for all comparison methods. If one compares to prior work, they should only compare to results that searched the same hyper-parameter space.
\end{theorem}


==> tables/data_split_figure_illustration.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{cv_mdl_ms.pdf}
    \caption{\small{Illustration of how different data split strategies partition the labelled data, with $K=4$ and $r=0.5$.}}
    \label{fig:datasplit}
\end{figure}
